DORE: An Experimental Framework to Enable Outband D2D Relay in Cellular Networks

Device-to-Device communications represent a paradigm shift in cellular networks. In particular, analytical results on D2D performance for offloading and relay are very promising, but no experimental evidence validates these results to date. This paper is the first to provide an experimental analysis of outband D2D relay schemes. Moreover, we design DORE, a complete framework for handling channel opportunities offered by outband D2D relay nodes. DORE consists of resource allocation optimization tools and protocols suitable to integrate QoS-aware opportunistic D2D communications within the architecture of 3GPP Proximity-based Services. We implement DORE using an SDR framework to profile cellular network dynamics in the presence of opportunistic outband D2D communication schemes. Our experiments reveal that outband D2D communications are suitable for relaying in a large variety of delay-sensitive cellular applications, and that DORE enables notable gains even with a few active D2D relay nodes.

==> architecture.tex <==
\section{Background: 3GPP ProSe Architecture for D2D Communication}
\label{s:background}

%%The outstanding outcome of the theoretic studies on D2D drove mobile operators and the 3GPP standardization body to consider the D2D paradigm as a system component for the next generation cellular standards. Indeed, 
%3GPP  is actively studying  the feasibility of D2D communications to provide users with services between radio neighbors, i.e., the aforementioned Proximity-based Services~(ProSe), using either {\it inband} or {\it outband} D2D techniques. These techniques are distinguished based on the communication spectrum and technology employed. Inband D2D uses the cellular interface and takes place in the cellular spectrum, while outband D2D uses a secondary interface (e.g., the WiFi interface) and  takes place in the unlicensed spectrum.
%
%A comprehensive state-of-the-art survey for D2D communications in~\cite{asadi2014survey} shows that the articles on inband D2D outnumber those of outband D2D. Indeed, a quick look at the state-of-the-art shows that inband D2D is a well-explored topic. Although its standardization is progressing slowly due to the significance of the required modifications for accommodating D2D users over the costly cellular spectrum. Hence, the community is moving its attention towards outband D2D to leverage the potentials of D2D communications as soon as possible~\cite{andreev2014ComMag}.
%
%
%%unlike outband D2D~\cite{asadi2013survey}. This is mostly due to the skepticism of the community accepting WiFi or similar technologies as platform for D2D communications in cellular networks. However, the latest release of 3GPP's technical reports~\cite{yyy} indicates that the standardization body considers both inband and outband techniques to be valid for D2D communication. 
%%However, the standardization progress for inband D2D is slow due to the significance of the required modifications for accommodating D2D users over cellular spectrum. Hence, the community is moving its attention towards outband D2D to leverage the potentials of D2D communications as soon as possible~\cite{andreev2014ComMag}.
%
%Despite the unavailability of the standardization for D2D communications, possible design could be mapped through the ongoing feasibility studies and technical reports that deal with D2D (see in particular~\cite{3GPP23.703, 3GPP23.303, 3GPP36.843}). 
%In the remainder of this section we give an overview of the 3GPP's D2D-enabled cellular network architecture profiled in ProSe. In addition, we detail the main network elements for ProSe-based D2D operation and their associated procedures. 

%Here, we introduce a few definitions before describing the 3GPP's envisioned architecture for D2D communications. 
%
%{\bf Application ID.} The network assigns a unique Application ID to each D2D service. It is used to identify the related ProSe Application Server. 
%
%{\bf Application User ID.} Each UE is given an Application User ID that is used to identify the UE at the ProSe Application Server.


%\subsection{ProSe functional elements}

There are three main elements for supporting D2D communications, namely, ProSe Application, ProSe Application Server, and ProSe Function (see Fig.~\ref{fig:proseArch}). 
%
The {\bf ProSe Application} runs at the UE. It handles the necessary D2D signaling and procedures at the UE side. For example, a given ProSe Application can send beacons to discover new nodes or it can also be discovered by sending the location information to the Evolved Packet Core (EPC).
%
The {\bf ProSe Application Server} provides the necessary functionalities for a given application. It also supports the application layer functionalities such as the storage of EPC ProSe User's IDs. 
%
The {\bf ProSe Function} is located inside EPC that acts as a reference point towards the ProSe Application Server, the EPC and the UE. ProSe Function manages procedures such as authorization, UE configuration, security, and billing.

\begin{figure} [t!]
\centering
		\includegraphics[scale=0.55, angle=0]{./figs/proseArch.pdf} %[width=70mm,angle=0] [scale=0.80, angle=0]
		\vspace{-2mm}
		\caption{3GPP's envisioned ProSe architecture.}
		\vspace{-4mm}
		\label{fig:proseArch}
\end{figure}

%\subsection{D2D related procedures in ProSe}
%The key procedures in D2D communications are Discovery and Direct Communication. 
%
%{\bf Discovery} is the procedure that allows a UE to discover another UE before the initiation of a communication. According to 3GPP, there are two types of discovery, namely, direct discovery and EPC-level discovery. In direct discovery, UE searches for other devices in proximity independent of the network. Here, the UEs use periodical beacon transmission/reception to communicate with other UEs. This approach is particularly beneficial in out-of-coverage scenarios where network assistance is no longer available. In EPC-level discovery, as the name suggests, the EPC keeps track of the UE's location and triggers the device discovery process upon detection of another UE in proximity. 
%This approach reduces the energy consumption at UE since the transmission of the discovery beacons is not required.
%
%Upon the completion of the discovery procedure between the UEs, the {\bf Direct Communication} is the procedure that allows inter-UE communications, which can be network-authorized or network-independent. Both methods support one-to-one, one-to-many, and relay use-cases. In addition, communication can occur inband (over the licensed spectrum) or outband (over unlicensed spectrum).
































==> testbed.tex <==
\section{SDR-based testbed for outband D2D communications}
\label{s:testbed}

In this section, we describe the hardware, the software, and the architecture of our testbed. Our testbed design is utterly beneficial because it is based on an SDR platform that uses Field Programmable Gate Array (FPGA) modules for high-speed Digital Signal Processing (DSP) prototyping. Moreover, it exploits the Real-time controllers  which ensures quick protocol prototyping. As today's cellular networks are moving toward functional virtualization and new architecture, SDR platforms certainly stand out among the prototyping alternative in today's market. 

%The testbed consists of two main elements, namely, the eNB and the UEs. We choose to use LabView for prototyping outband D2D because LabVIEW FPGA allows us to implement high speed DSP operations (e.g.,FFT, iFFT, encoding, and decoding) in FPGA. In addition, operations such as scheduling can be implemented quickly using LabVIEW Real-Time.

\subsection{Software and hardware}
{\bf Software.} We found LabVIEW\footnote{http://www.ni.com/labview/} as a suitable tool to prototype an outband D2D platform. On one hand, LabVIEW FPGA allows for quick implementation of computationally intensive Physical layer (PHY) operations (e.g., Fast Fourier Transform (FFT), inverse FFT (iFFT), encoding, and decoding) in Xilinx FPGA and meets the stringent nano-second time scale requirement of the digital communication systems. Moreover, it provides the necessary means for high speed communication with CPU/RF hardware. On the other hand, LabVIEW Real-Time is suitable for implementing MAC layer operations with micro-second resolution. LabVIEW Real-Time runs on a general purpose CPU and communicates with LabVIEW FPGA over high-speed PCIe backplane.

{\bf Hardware.} The hardware used in this testbed is NI PXI 1082 chassis\footnote{http://sine.ni.com/nips/cds/view/p/lang/en/nid/207346} that contains: $(i)$ NI PXIe 8135 Real-Time controller\footnote{http://sine.ni.com/nips/cds/view/p/lang/en/nid/210545} operating on an Intel Core-i7-3610QE CPU. This controller is used to execute LabVIEW Real-Time which runs MAC layer algorithm and physical layer control algorithms. LabVIEW Real-time communicates with the FPGA through dedicated Direct Memory Access (DMA) FIFOs; $(ii)$ The Physical layer is programmed using LabVIEW FPGA and runs on NI FlexRIO modules\footnote{http://www.ni.com/flexrio/} that are equipped with Xilinx Kintex 7 or Virtex 5 FPGAs; $(iii)$ NI 5791 FlexRIO Adaptor Module (FAM) is used as an RF transceiver operating with a $200$ MHz bandwidth the in frequency range $200$ MHz to $4.4$ GHz. This is used for Digital to Analog Conversion (DAC), Analog to Digital Conversion (ADC), up-converting  base-band to band-pass, and down-converting band-pass to base-band. 

%Fig.~\ref{fig:hardware} illustrates all these components. 
%\begin{figure} [t!]
%\centering
%		\includegraphics[scale=0.35, angle=0]{./figs/hardware.pdf} %[width=70mm,angle=0] [scale=0.80, angle=0]
%		\caption{Illustration of the hardwares used for the testbed.}
%		\label{fig:hardware}
%\end{figure}

\subsection{Architecture of eNB}
The eNB consists of a Real-Time controller and a FlexRIO module used for over the air LTE transmission. 
Fig.~\ref{fig:eNB} shows the important blocks of the eNB. Real-Time controller runs MAC layer services such as scheduling, D2D services, and Transport Block (TB) generation for Control Channel (CCH) and shared channel (SCH). FPGA executes PHY operations such as convolutional coding, interleaving for CCH traffic and scrambling for SCH traffic. Finally, the base-band signal is up-converted in the FAM module and transmitted to the UE over the air. The current testbed only supports OFDMA in downlink and the uplink transmissions is performed  over ethernet. However, in future we intend to extend this testbed to support OFDMA uplink transmission.
 

\begin{figure} [t!]
\centering
		\includegraphics[scale=0.40, angle=0]{./figs/eNB.pdf} %[width=70mm,angle=0]  [scale=0.80, angle=0]
		\caption{Architecture of the eNB.}
		\label{fig:eNB}
		\vspace{-5mm}
\end{figure}


\subsection{Architecture of UE}
As eNB only requires one interface, UE's architecture is thus more complex since it comprises of two interfaces: $(i)$~an LTE OFDMA downlink receiver for communicating with the eNB; and $(ii)$ a WiFi transceiver to establish the outband D2D link with other UEs. 

{\bf OFDMA receiver.}  Following the design  of the transmitter, the DSP operations are implemented in the FPGA. Real-Time controller is only used for processing the received payload and MAC layer D2D operations. These operations mainly consist in filtering the relay packets and transmitting them to the WiFi interface for relaying.  Fig.~\ref{fig:UE-lte} shows the location of different logical blocks in the system.

\begin{figure} [h!]
\centering
		\includegraphics[width=0.87\columnwidth, angle=0]{./figs/UE-lte.pdf} %[width=70mm,angle=0] [scale=0.80, angle=0]
		\caption{Architecture of UE's LTE interface.}
		\label{fig:UE-lte}
\end{figure}

{\bf WiFi transceiver.} The majority of the WiFi framework~\cite{wifi2014NI} is implemented in FPGA. In addition, the transceiver is implemented within the same FPGA. We implemented the D2D state-machine and its corresponding logic in the Real-Time controller. The controller is also in charge of feeding data to the FPGA transmission processing chain and reading the decoded data from FPGA reception processing chain. 
Fig.~\ref{fig:UE-wifi} shows the structure of the WiFi framework.



\begin{figure} [t!]
\centering
		\includegraphics[width=0.85\columnwidth, angle=0]{./figs/UE-wifi.pdf} %[width=70mm,angle=0] [scale=0.80, angle=0]
		\caption{Architecture of UE's WiFi interface.}
		\vspace{-5mm}
		\label{fig:UE-wifi}
\end{figure}



